Decorrelate Irrelevant, Purify Relevant: Overcome Textual Spurious Correlations from a Feature Perspective

Natural language understanding (NLU) models tend to rely on spurious correlations (i.e., dataset bias) to achieve high performance on in-distribution datasets but poor performance on out-of-distribution ones. Most of the existing debiasing methods often identify and weaken these samples with biased features (i.e., superficial surface features that cause such spurious correlations). However, down-weighting these samples obstructs the model in learning from the non-biased parts of these samples. To tackle this challenge, in this paper, we propose to eliminate spurious correlations in a fine-grained manner from a feature space perspective. Specifically, we introduce Random Fourier Features and weighted re-sampling to decorrelate the dependencies between features to mitigate spurious correlations. After obtaining decorrelated features, we further design a mutual-information-based method to purify them, which forces the model to learn features that are more relevant to tasks. Extensive experiments on two well-studied NLU tasks demonstrate that our method is superior to other comparative approaches.

==> outline/discussion.tex <==
\section{Discussion}


% 1) Novelty is not enough.
% Specifically, from my understanding, this paper applies and validates the approach of ["Deep stable learning for out-of-distribution generalization." CVPR2021] as "feature decorrelation" phase on natural-language-related datasets rather than vision-related datasets (even almost large sections of assumptions, formulas, and derivations in section 3.1 are the same as CVPR2021), and moreover introducing mutual information as "feature purification" phase. Could authors highlight the differences and contributions of DePro compared to the [CVPR2021]?


% 在这一小节中，我们主要讨论两件事情，1）为什么我们使用RFF对特征进行节藕(disentanglement\disentangle)。2）我们和其他使用RFF对特征进行解耦的文章的区别。
In this section, we primarily discuss two aspects: 1) Why we choose RFF as the feature disentanglement method; 2) What distinguishes this work from prior works that use RFF to decouple features. 
% 有很多工作\cite{rahimi2007random, zhang2021deep, DBLP:journals/corr/KingmaW13, HigginsMPBGBML17}提出提高模型的鲁棒性by performing latent representation disentanglement learning.

Many works \cite{rahimi2007random, zhang2021deep, DBLP:journals/corr/KingmaW13} have been proposed to improve the robustness of the model by performing latent representation disentanglement learning. We compared the performance of two disentanglement methods RFF\cite{rahimi2007random} and $\beta$-VAE\cite{DBLP:conf/iclr/HigginsMPBGBML17} in our model structure. The performance results are illustrated in \ref{vaerff}, which shows that RFF outperforms $\beta$-VAE in our model both in ID and OOD datasets. In contrast to RFF, VAE disentangles the representation while compressing it, thus damaging the generalization ability. So we choose RFF to disentangle the feature representation to obtain the uncompressed disentangled representation, which benefits succeeding feature purification to distinguish useful from useless local features.
% 我们也比较了RFF\cite{???}和$\beta$-VAE\cite{???}两个结偶方法在我们的模型结构上的表现。
% 两个方法在NLI task和FV task上的表现如\ref{tab:vae_rff}，可以发现在我们的结构中使用rff对特征进行结偶可以具有更好的表现无论是在ID datasets还是在OOD datasets。
% 相比较于RFF，VAEs在对表示进行节藕的同时，还对表示进行了压缩从而损失了一定的泛化特征，而RFF不会对表示进行压缩，所以我们使用RFF对表示进行节藕，可以获得未经过压缩的disentangled的表示，从而更有利于在后续进行feature提纯，来区分有用和无用的local feature。


% 本文的第一个阶段（i.e., 3.1 feature decorrelation）确实主要参考了这篇文章的方法，同时在section 3.1中也多次引用了这篇文章。
% The first phase of our proposed method (i.e., 3.1 feature decorrelation) did refer primarily to the method of [2], and it was also referenced several times in section 3.1.
% 本文DePro和这篇文章的主要区别在于，本文不仅仅使用RFF对特征进行去相关。我们将对特征处理的两个相辅相成的方法（i.e., 特征去相关和特征提纯）相互结合。
The distinction between \emph{DePro} and other RFF-based methods is that our method not only uses RFF for feature decoration but also combines two complementary approaches (i.e., feature decorrelation and feature purification).
% 特征去相关和特征提纯并不是相互独立的两个方法。在4.3 Ablation Study 中我们也详细分析了二者的关系，即去相关后的特征能够更好的被提纯，让模型在提纯有用特征时更多的忽略其中的杂质（i.e., 无关特征）。
These two methods are not mutually exclusive. In \ref{sec:Sensitivity}, we analyzed the relationship between these two in detail, that is, the decorrelated features can be better purified, allowing the model to ignore more impurities when purifying useful features.
% 同时特征提纯能够约束模型关注去相关后的有用特征，更少的关注无用特征。
Moreover, after feature decorrelation, feature purification can constrain the model to concentrate more on useful features rather than useless features.
% 所以本文贡献之一是首次将这两个相关的方法自然的融合在一起。
% 同时本文更多的贡献在Review 2, Question 1被提到。
% So one of the contributions of our paper is the first time proposing the natural fusion of these two related methods.
% Moreover, more contributions to our paper are mentioned in Review 2, Question 1 and section 1 Introduction.


% % 正如您所说，这个框架不仅仅局限于NLU的debias任务，在NLP中大部分基于预训练模型的任务都可以尝试使用本文提出的框架来提高各种NLP任务的表现，
% % 我们也将在未来工作中尝试将这个框架应用在不同任务中。
% % 同时也希望这篇文章能够启发NLP community中更多的人尝试本文提出的两个相辅相成的关于特征处理的方法。
% As for the generalization of our proposed method, it is not only limited to the debias task of NLU, most of the tasks in NLP can try to use the framework our proposed to improve the performance of various NLP tasks.
% We will also try to apply this framework to different tasks in our future work.
% % Moreover, I hope that this article can inspire more people in the NLP community to try the two complementary methods on feature processing proposed in this article.

% %[Zhang et al., 2021] Xingxuan Zhang, Peng Cui, Renzhe Xu, Linjun Zhou, Yue He, and Zheyan Shen. Deep stable learning for out-of-distribution generalization. In CVPR, pages 5372–5382, 2021.


